Confidence v.s. Critique: A Decomposition of Self-Correction Capability for LLMs

Large Language Models (LLMs) can correct their self-generated responses, but a decline in accuracy after self-correction is also witnessed. To have a deeper understanding of self-correction, we endeavor to decompose, evaluate, and analyze the self-correction behaviors of LLMs. By enumerating and analyzing answer correctness before and after self-correction, we decompose the self-correction capability into confidence (being confident to correct answers) and critique (turning wrong answers to correct) capabilities, and propose two metrics from a probabilistic perspective to measure these 2 capabilities, along with another metric for overall self-correction capability evaluation. Based on our decomposition and evaluation metrics, we conduct extensive experiments and draw some empirical conclusions. For example, we find different models can exhibit distinct behaviors: some models are confident while others are more critical. We also find the trade-off between the two capabilities (i.e. improving one can lead to a decline in the other) when manipulating model self-correction behavior by prompts or in-context learning. Further, we find a simple yet efficient strategy to improve self-correction capability by transforming Supervision Fine-Tuning (SFT) data format, and our strategy outperforms vanilla SFT in both capabilities and achieves much higher accuracy after self-correction. Our code will be publicly available on GitHub.

==> content/Methodology_past.tex <==
% 问题的形式化定义，数学符号
% 评测的指标
% 概率估计的方法
% 指标收敛性分析

% 通过章节1的分析，我们把LLM 的self-correction capability分解为了对正确答案的自信程度和对错误答案的反思能力。为了进一步去分析模型的这两种能力，首先我们形式上规范化模型自我纠正这一过程并引入相关的数学符号，然后我们从概率的角度分别提出两个指标来measure模型的这两种能力。接下来，我们证明了模型自我纠正之后的表现（即准确率），本质上是上述两个指标的加权求和。由于我们指标的计算依赖于事件的概率，我们又给出了相应事件的概率估计方法，以及分析了指标的收敛性。
\label{sec:methodology}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.48\textwidth]{fig/Venn.pdf}
    \caption{.}
    \label{fig:Venn}
\end{figure}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.48\textwidth]{fig/RCS.pdf}
    \caption{.}
    \label{fig:RCS} 
\end{figure}

In \S \ref{sec:decomposition}, we have decomposed the self-correction capability of LLMs into two distinct aspects: the confidence level in correct answers and the reflective ability regarding incorrect answers. To further investigate these capabilities, we first formalize the process of model self-correction and introduce relevant mathematical notations (\S \ref{subsec:notations}). Then we propose two metrics from a probabilistic perspective to measure these two capabilities (\S \ref{subsec:confidence} and \S \ref{subsec:refection}). Subsequently, we demonstrate that model performance after self-correction (i.e., accuracy) is essentially a weighted sum of the aforementioned two metrics (\S \ref{subsec:weighted_sum}). Since the computation of our metrics depends on the probability of events, we then provide probability estimation methods and analyze the convergence properties of the metrics (\S \ref{subsec:probability_estimation}).

\subsection{Notations}
\label{subsec:notations}
Initially, we have a set comprising of $n$ questions, denoted as $A = \{ a_1, a_2, ..., a_n \}$. For a given question $a_i$, we ask the model twice: (1) in the first round, we directly ask question $a_i$ and the model generates a correct answer through a single temperature-based sampling with probability $P(a_i)$; (2) After asking the model question $a_i$ and getting a model-generated answer (no matter correct or wrong), we challenge this model and ask the model to answer the question again, and model generate correct answer with probability $P(b_i)$. We define the following stochastic process: 

\textbullet~ \textit{Randomly sampling a question $a_i$ from $A$ with equal probability and asking the model twice according to the above procedure.} 

In the above random process, the probability of the model generating a correct answer in round 1 and round 2 is denoted as $P(a)$ and $P(b)$, respectively. We define their expectations as accuracy1 and accuracy2 (acc1 and acc2 for short):

\begin{equation}
acc1 = E[P(a)] = \frac{\sum_{i=1,...,n}P(a_i)}{n} 
\end{equation}

\begin{equation}
acc2 = E[P(b)] = \frac{\sum_{i=1,...,n}P(b_i)}{n} 
\end{equation}

\subsection{Confidence Level}
\label{subsec:confidence}
How confident are language models to their correct answers? To answer this question from a probabilistic perspective, we introduce a metric named \textbf{C}onfidence \textbf{L}evel (\textbf{CL}), which is the conditional probability of a model generating a correct answer in round 2 given it has generated a correct in round 1.
Initially, the prior probability of selecting $a_i$ in the above random process is $P(select \  a_i) = \frac{1}{n}$. After introducing the condition that the model has answered question $a_i$ correctly in round 1, the posterior probability of $a_i$ being selected in the random process becomes $P(select \  a_i) = \frac{P(a_i)}{\sum_{j=1,...,n}P(a_j)}$. By leveraging this posterior probability for the calculation of expected values, we have:

\begin{equation}
\label{equ:CL}
\begin{aligned}
CL &= E[P(b|a)] \\
&= \sum_{i=1,...N}P(select \  a_i)P(b_i|a_i) \\
&= \sum_{i=1,...,n}\frac{P(a_i)}{\sum_{j=1,...,n}P(a_j)}P(b_i|a_i) \\
&= \frac{\sum_{i=1,...,n}P(a_i)P(b_i|a_i)} {\sum_{i=1,...,n}P(a_i)},
\end{aligned}
\end{equation}

where $P(b_i|a_i)$ is the conditional probability of a model correctly answering $a_i$ in round 2 given that it has correctly answered it in round 1. The higher CL is, the more confident the model is about its correct answers. High CL also indicates the model is confident and will not change its correct answer even when challenged.

\subsection{Correction Capability}
\label{subsec:refection}
% Can language models correct their answers after making mistakes in round 1? 
After being challenged, can language models be aware of their mistakes in round 1 and willing to correct them in round 2?
To answer this question from a probabilistic perspective, we introduce a metric named \textbf{C}orrection \textbf{C}apability (\textbf{CC}), which is the condition probability of a model giving a correct answer in round 2 given 
that it has answered the question incorrectly in round 1. We can derive CC in a manner similar to Equation \ref{equ:CL}, but here we would give another form of derivation:

\begin{equation}
\begin{aligned}
CC &= E[P(b|\neg a)] \\
&= E[\frac{P(b,\neg a)}{P(\neg a)}] \\
&= \frac{\sum_{i=1,...,n}P(b_i,\neg a_i)/N}{\sum_{i=1,...,n}P(\neg a_i)/N} \\
&= \frac{\sum_{i=1,...,n}P(b_i|\neg a_i)P(\neg a_i)}{\sum_{i=1,...,n}P(\neg a_i)} \\
&= \frac{\sum_{i=1,...,n}[1-P(a_i)]P(b_i|\neg a_i)}{\sum_{i=1,...,n}[1-P(a_i)]},
\end{aligned}
\end{equation}

where $P(b_i|\neg a_i)$ is the conditional probability of a model correctly answering $a_i$ in round 2 given that it has answered it wrong in round 1, and model answer $a_i$ wrong with probability $P(\neg a_i) = 1 - P(a_i)$. 
CC reflects the extent to which the model persists in providing wrong answers. A lower CC value indicates a greater tendency for the model to stubbornly maintain erroneous responses, whereas a higher CC value suggests a greater willingness of the model to correct these errors.
% CC这个指标反映了模型对错误答案的固执程度，CC值越低说明模型越会固执的坚持错误答案，而更高的CC值则说明模型在愿意纠正错误答案。


\subsection{What Makes High Acc2?}
\label{subsec:weighted_sum}
%怎么让模型在被质疑后仍有较高的准确率呢？概率分解公式有$P(b_i)=P(b_i|a_i)P(a_i)+P(b_i|\neg a_i)P(\neg a_i)$。
% 模型在第一轮做对的条件下，第二轮越能对自己的答案越自信，就越不容易更改答案，从而第二轮就更容易也做对。模型在第一轮做错的情况下，模型能够更正错误答案，第二轮也就更容易做对。基于这两点，直观上来说更高的CL值和CC值都会导致更高的acc2。我们同样发现他们有下面数学关系：

How can we ensure that a model maintains a high accuracy even after being challenged? According to the probability decomposition formula, we have  $P(b_i)=P(b_i|a_i)P(a_i)+P(b_i|\neg a_i)P(\neg a_i)$, which indicates: 
(1) In the scenario where the model provides a correct answer in round 1,
high model confidence in its answer will lead to low likelihood of changing its response, and consequently results in a high probability of correctness in round 2;
(2) Conversely, if the model initially provides an incorrect answer, it has the opportunity to correct its error in the second round, which also facilitates a higher likelihood of providing a correct answer.


Based on these observations, it can be intuitively concluded that higher values of $CL$ and $CC$ will lead to an increase in $acc2$. Besides, we also discover the following mathematical relationships:

\begin{equation}
\begin{aligned}
& acc2 \\
&= \frac{\sum_{i=1,...,n}P(b_i)}{n} \\ 
&= \frac{\sum_{i=1,...,n}P(b_i|a_i)P(a_i)+P(b_i|\neg a_i)P(\neg a_i)}{n} \\
&= \frac{\sum_{i=1,...,n}P(a_i)}{n}\frac{\sum_{i=1,...,n}P(a_i)P(b_i|a_i)}{\sum_{i=1,...,n}P(a_i)} \\
& + \frac{\sum_{i=1,...,n}[1-P(a_i)]}{n}\frac{\sum_{i=1,...,n}P(\neg a_i)P(b_i|\neg a_i)}{\sum_{i=1,...,n}[1-P(a_i)]} \\
&=acc1*CL+(1-acc1)*CC
\end{aligned}
\end{equation}

% 本质上来说，acc2是CL和CC分别以权重acc1和(1-acc1)的加权求和。换句话说，如果固定acc1不变，模型第二轮的准确率和CL和CC分别呈现出线性正相关。
Essentially, $acc2$ is the weighted sum of $CL$ and $CC$ with weights $acc1$ and $1 - acc1$, respectively. In other words, assuming $acc1$ remains constant, accuracy in round 2 exhibits a linear positive correlation with both $CL$ and $CC$.



\subsection{Probability Estimation}
\label{subsec:probability_estimation}
% 分类任务用logits+softmax来估计概率
% 生成任务用多次采样的方式来估计概率
% 上述的两个指标都是从概率的角度去推导得到的，指标的计算也依赖于这些P(a)等。然而，实际值P(a)是无法得到的，在实际实验中，我们用数理统计的方法去得到估计值P(a^)来代替这些真实值完成指标计算。目前NLP任务主要分为分类任务和生成任务，我们将分别去讨论这两类任务上的概率估计方法。

% 分类任务：对于一个K分类任务，我们记所有候选label的集合为$L = \{label_0,label_2,...,label_{K-1}\}$(例如，对于MMLU任务来说，候选集$L=\{A,B,C,D\}$). 语言模型在做next-token prediction时，会先得到一个logit向量$（）$，其中每一个值对应词表上一个词的logit值,$｜V｜$表示词表的尺寸，然后把logits向量输入softmax层得到词表上下一个词的概率分布。我们在做分类任务时，只关心所有候选label的概率分布，而不关心词表上其他词的概率分布，所以我们把logit向量中其他词丢弃，只保留候选label对应的词进而得到一个精简后的logit 向量，然后过softmax层之后得到模型预测每个label对应的概率$P(l_0),P(l_1),...,P(l_{K-1})$. 不失一般性，我们不妨假设正确的label是$l_0$,那么我们有$P(a^)=P(l_0)$。我们再测试一下给定模型正确的label $l_0$的条件下，模型self-correct之后给出的label候选集上的概率分布$P(l_0)｜l_0,P(l_1｜l_0),...,P(l_{K-1}｜l_0)$, 然后有$P(b|a^)=P(l_0|l_0)$. 对于$P(b|\neg a)$的计算则较为复杂，我们需要分别把每个错误的label $l_j (j!= 0)$给模型，分别让模型进行自我纠正，并得到把该错误改正为正确label $l_0$的概率$P(l_0|l_j)$. 最后我们用概率展开公式得到$P(b|\not a) = \Sum P(l_0|l_j)P(l_j)$。

% 生成任务：我们用多次采样，观察到正确和错误答案的频率来估计概率。对于一个问题$q_i$, 我们直接问模型该问题，得到答案后再让模型自我修正该答案，得到最终答案。我们把这个过程重复$T$次，并统计每对答案的正确性，最终得到序列$(a_i^0,b_i^0),(a_i^1,b_i^1),\ldots, (a_i^{T-1},b_i^{T-1})$，其中$(a_i^t,b_i^t)$表示第$t$次重复实验的结果，他们分别指示了自我纠正前后答案的正确性（如果初试答案正确则$a_i^t=1$，错误则$a_i^t=1$；$b_i^t=1$同理）。利用频率估计概率我们有：（1）$\hat{P}(a_i) = \frac{\sum_{t=0}^{T-1}a_i^t}{T}$; (2) $\hat{P}(b_i|a_i) = \frac{\sum_{t=0,\ldots,T-1}a_i^t b_i^t}{\sum_{t=0,\ldots,T-1}a_i^t}$; (3) $\hat{P}(b_i|\neg a_i) = \frac{\sum_{t=0,\ldots,T-1}(1-a_i^t)b_i^t}{\sum_{t=0,\ldots,T-1} 1-a_i^t}$ .

The above two metrics are derived from a probabilistic perspective, and their calculation relies on 3 key probability values \( P(a_i), P(b_i|a_i) \) and \( P(b_i| \neg a_i) \) of each question $q_i$. However, the actual values of these probabilities are unattainable. In practice, we utilize statistical methods to obtain their estimates \( \hat{P}(a), \hat{P}(b_i|a_i) \) and \( \hat{P}(b_i| \neg a_i) \) to substitute these true values for metric computation.
Currently, natural language processing (NLP) tasks can be generally divided into classification tasks and generation tasks, and we will discuss the probability estimation methods applied to these two types of tasks separately.

\paragraph{Probability Estimation for Classification Tasks.} For a \( K \)-class classification task, let the set of all candidate labels be denoted as \( L = \{l_0, l_1, \ldots, l_{K-1}\} \) (e.g., for the MMLU, the candidate set is \( \{A, B, C, D\} \)). A question $q_i$ is fed into the model and the model is asked to output the predicted label. When the model performs next-token prediction, it first generates a logit vector $(o_0,o_1,...o_{|V|})$, where each value corresponds to the logit of a token in the vocabulary \(V\) and \(|V|\) denotes the size of the vocabulary. In the generation process, The logit vector is then passed through a softmax layer to produce the probability distribution of the next token in the whole vocabulary.
However, for classification tasks, we are only interested in the probability distribution over candidate label set $L$ instead of vocabulary $V$. Therefore, we discard most logit values, retaining only those corresponding to candidate labels, resulting in a reduced logit vector $(o^{'}_0, o^{'}_1, \ldots, o^{'}_{K-1})$. After applying the softmax layer, the model predicts the probability for each label \( P(l_0), P(l_1), \ldots, P(l_{K-1}) \). 

(1). Without any loss of generality, assume the correct label is \( l_0 \), then we have \( \hat{P}(a_i) = P(l_0) \).

(2). Next, we feed the correct answer \( l_0 \) into the model and ask the model to self-correct. The model outputs the probability distribution over candidate labels, denoted as \( P(l_0|l_0), P(l_1|l_0), \ldots, P(l_{K-1}|l_0) \), then we have \( \hat{P}(b_i|a_i) = P(l_0|l_0) \).

(3). The computation of \( \hat{P}(b_i|\neg a_i) \) is more complex. For each incorrect label \( l_j \) (\( j \neq 0 \)), we input it to the model and allow for self-correction, obtaining the probability of correcting it to the correct label \( P(l_0|l_j) \). Finally, by using the law of total probability, we have \( \hat{P}(b_i|\neg a_i) = \sum_{j=1,\ldots,K-1} P(l_0|l_j)P(l_j) \).


\paragraph{Probability Estimation for Generation Task.} We employ multiple sampling to estimate probabilities by observing the frequency of correct and incorrect answers. Given a question \(q_i\), we pose it to the model and obtain an initial answer. Subsequently, the model is prompted to self-correct the initial answer, resulting in a final answer. This process is repeated \(T\) times, and for each pair of initial and final answers, we evaluate their correctness. This yields a sequence of results \((a_i^0, b_i^0), (a_i^1, b_i^1), \ldots, (a_i^{T-1}, b_i^{T-1})\), where \((a_i^t, b_i^t)\) denotes the outcome of the \(t\)-th repetition. Specifically, \(a_i^t\) and \(b_i^t\) indicate the correctness of the initial and final answers, respectively. For a correct initial answer, \(a_i^t = 1\); otherwise, \(a_i^t = 0\) and The same logic applies to \(b_i^t\). Utilizing frequency to estimate probability, we have: 

(1). \(\hat{P}(a_i) =  \frac{\sum_{t=0}^{T-1}a_i^t}{T}\);

(2). \(\hat{P}(b_i|a_i) = \frac{\sum_{t=0}^{T-1} a_i^t b_i^t}{\sum_{t=0}^{T-1} a_i^t}\);

(3). \(\hat{P}(b_i|\neg a_i) = \frac{\sum_{t=0}^{T-1} (1-a_i^t)b_i^t}{\sum_{t=0}^{T-1} (1-a_i^t)}\)

% These calculations facilitate an understanding of the model's performance regarding its capability to self-correct initial errors.










